Graph Self-supervised Learning with Accurate Discrepancy Learning

Self-supervised learning of graph neural networks (GNNs) aims to learn an accurate representation of the graphs in an unsupervised manner, to obtain transferable representations of them for diverse downstream tasks. Predictive learning and contrastive learning are the two most prevalent approaches for graph self-supervised learning. However, they have their own drawbacks. While the predictive learning methods can learn the contextual relationships between neighboring nodes and edges, they cannot learn global graph-level similarities. Contrastive learning, while it can learn global graph-level similarities, its objective to maximize the similarity between two differently perturbed graphs may result in representations that cannot discriminate two similar graphs with different properties. To tackle such limitations, we propose a framework that aims to learn the exact discrepancy between the original and the perturbed graphs, coined as Discrepancy-based Self-supervised LeArning (D-SLA). Specifically, we create multiple perturbations of the given graph with varying degrees of similarity, and train the model to predict whether each graph is the original graph or the perturbed one. Moreover, we further aim to accurately capture the amount of discrepancy for each perturbed graph using the graph edit distance. We validate our D-SLA on various graph-related downstream tasks, including molecular property prediction, protein function prediction, and link prediction tasks, on which ours largely outperforms relevant baselines.

==> tables/analysis.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{lcc}
        \toprule
        Dataset & Act. Sim. & Inact. Sim. \\
        \midrule
        BACE    & \textbf{0.6743} & \textbf{0.5403} \\
        \midrule
        BBBP    & 0.3961 & 0.2031 \\
        ClinTox & 0.2724 & 0.2278 \\
        HIV     & 0.4186 & 0.4536 \\
        MUV     & 0.1946 & 0.4181 \\
        SIDER   & 0.2880 & 0.2316 \\
        Tox21   & 0.3047 & 0.3462 \\
        ToxCast & 0.2193 & 0.2962 \\
        \bottomrule
    \end{tabular}
    \caption{Comparison of Tanimoto similarity on benchmark datasets of chemical domain. The reported values are top-5 similar molecules with an anchor molecule.}
    \label{tab:analysis}
\end{table}

==> tables/link_pred.tex <==
\begin{table}[t]
\centering
    \begin{adjustbox}{width=\columnwidth}
    \begin{tabular}{lccc|c}
    \toprule
    SSL Method & COLLAB & IMDB-B & IMDB-M & Avg. \\
    \midrule
    No Pretrain  & 84.53 $\pm$ 0.55 & 72.54 $\pm$ 1.11 & 70.25 $\pm$ 1.49 & 71.33 \\
    \midrule
    \multicolumn{3}{l}{\textit{Predictive learning}} \\
    AttrMasking  & 85.07 $\pm$ 0.49 & 73.84 $\pm$ 1.11 & 70.26 $\pm$ 1.62 & 72.32 \\
    ContextPred  & 86.49 $\pm$ 0.35 & 72.04 $\pm$ 1.24 & 66.99 $\pm$ 1.63 & 69.95 \\
    \midrule
    \multicolumn{3}{l}{\textit{Contrastive learning}} \\
    Infomax      & 83.13 $\pm$ 0.35 & 68.46 $\pm$ 1.06 & 64.31 $\pm$ 4.07 & 67.59 \\
    GrpahCL      & 83. $\pm$ 0.85 & 67.44 $\pm$ 2.07 & 67.47 $\pm$ 2.81 & 67.48 \\
    JOAO         & 68.04 $\pm$ 0.97 & 68.82 $\pm$ 1.80 & 68.70 $\pm$ 0.66 & 68.52 \\
    GrpahLoG     & 72.94 $\pm$ 0.38 & 72.56 $\pm$ 2.09 & 70.59 $\pm$ 1.31 & 72.03 \\
    \midrule
    D-SLA~(Ours) & \textbf{76.19} $\pm$ 0.50 & \textbf{75.92} $\pm$ 1.65 & \textbf{72.97} $\pm$ 2.51 & \textbf{75.03}\\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Performance comparison of link prediction on social network of TU Dataset. The reported value is the average of accuracy of correct link prediction and the bold value is the best performance on each dataset.}
    \label{tab:link_pred}
\end{table}

==> tables/spearman_rank.tex <==
\begin{table}[t]
\centering
    \begin{adjustbox}{width=0.5\columnwidth}
    \begin{tabular}{lc}
    \toprule
    Method & Coefficient Avg. \\
    \midrule
    EdgePred    & 0.7163 $\pm$ 0.2793 \\
    AttrMasking & 0.8057 $\pm$ 0.2035 \\
    ContextPred & 0.7590 $\pm$ 0.2746 \\
    Infomax     & 0.6865 $\pm$ 0.2760 \\
    JOAO        & 0.6605 $\pm$ 0.3819 \\
    GraphLoG    & 0.8111 $\pm$ 0.1802 \\
    \midrule
    D-SLA~(Ours)& \textbf{0.9224} $\pm$ 0.1198 \\ 
    
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Rank correlation coefficient of 1000 graphs sampled from ZINC15. The graphs are perturbed with different strength and the rank correlation coefficient is measured by spearman's method. The right-end column~(vs. D-SLA) corresponds to the percentage of graphs with higher coefficient than the D-SLA's.}
    \label{tab:rank_coeff}
\end{table}
